Modelling informational entropy

By 'informational entropy', we understand an inherent boundary to knowability, due e.g. to perceptual, theoretical, evidential or linguistic limits. In this paper, we discuss a logical framework in which this boundary is incorporated into the semantic and deductive machinery, and outline how this framework can be used to model various situations in which informational entropy arises.

==> packages.tex <==
\usepackage{lscape}
\usepackage{pdflscape}

\usepackage{stmaryrd}

%\usepackage[greek.ancient,english]{babel}
%\usepackage[greek,english]{babel}

\usepackage{cmll}
\usepackage[table]{xcolor}
\usepackage{comment}

\usepackage{mathdots}

\usepackage{amscd}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathptmx}
\usepackage{mathrsfs}
\usepackage{color}
\usepackage{xspace}
\usepackage{bussproofs}
\EnableBpAbbreviations

\usepackage{tikz}

\usepackage{txfonts}

%\usepackage{bpextra}

%\usepackage{enumerate}

\usepackage{centernot}

\usepackage{mathtools}


\usepackage{relsize}

%\usepackage{caption}

\usepackage{multirow}

\usepackage{multicol}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{L}[1]{>{\arraybackslash}p{#1}}

%\usepackage{hyperref}[hyperfootnotes=false]
\usepackage{hyperref}
%\usepackage{cleveref}


